Federated Learning in Offline and Online EMG Decoding: A Privacy and Performance Perspective

Neural interfaces offer a pathway to intuitive, high-bandwidth interaction, but the sensitive nature of neural data creates significant privacy hurdles for large-scale model training. Federated learning (FL) has emerged as a promising privacy-preserving solution, yet its efficacy in real-time, online neural interfaces remains unexplored. In this study, we 1) propose a conceptual framework for applying FL to the distinct constraints of neural interface application and 2) provide a systematic evaluation of FL-based neural decoding using high-dimensional electromyography (EMG) across both offline simulations and a real-time, online user study. While offline results suggest that FL can simultaneously enhance performance and privacy, our online experiments reveal a more complex landscape. We found that standard FL assumptions struggle to translate to real-time, sequential interactions with human-decoder co-adaptation. Our results show that while FL retains privacy advantages, it introduces performance tensions not predicted by offline simulations. These findings identify a critical gap in current FL methodologies and highlight the need for specialized algorithms designed to navigate the unique co-adaptive dynamics of sequential-user neural decoding.

==> sections/sec_background.tex <==
\section{Federated Learning Background}

\subsection{Privacy For Biosignals}

\rev{
A foundational challenge in data privacy is mitigating linkability and identifiability, two of the seven core threats in the LINDDUN privacy threat modeling framework \cite{Priv_LINDDUN}. Linkability is an adversary's ability to distinguish whether items of interest (e.g., medical records, model weights, etc.) originate from the same source (e.g., a user). Linkability often serves as a precursor to identifiability, or the ability to uniquely identify a subject within a system \cite{Priv_LINDDUN, Priv_KAnon}. 
This progression from linkability to identifiability was famously demonstrated by Sweeney \cite{Priv_KAnon}, who showed that even when direct identifiers (e.g., names, SSNs) are removed, unique patterns in seemingly anonymized metadata (i.e., birth date, gender, and ZIP code) can be used to uniquely re-identify individuals by linking partially overlapping datasets. In the context of biosignals, this suggests that the privacy of a system depends not only on the protection of raw data, but also on the uniqueness of the metadata (e.g., summary statistics, model weights) that are stored or transmitted.

High-dimensional non-invasive neural signals, including electroencephalography (EEG), electrocardiogram (ECG), and electromyography (EMG), are increasingly recognized for encoding unintended sensitive attributes that machine learning models can extract \cite{Priv_HiddenInfoInBios, Priv_BiosPatientID}. Prior research has demonstrated that from these signals, model can estimate demographic traits like sex and age \cite{Priv_ECGAgeSexEstimation}, detect underlying medical conditions such as depression \cite{Priv_BehavioralPrivRisks}, and uniquely identify individuals \cite{Priv_EEGPersonIdentification, Priv_SecretFromEMG, Priv_EMGFeatDis, Priv_EMGPersIdentModels}. 
EMG data presents a significant re-identification risk because it encodes distinctive motor behaviors inherent to the individual. While these biometric markers enable secure applications like device authentication and pairing \cite{Priv_SecretFromEMG, Priv_EMGFeatDis}, they can likewise be exploited for record linkage or impersonation attacks. Recent studies underscore this threat, demonstrating that deep learning models can perform re-identification or impersonate users directly from surface EMG data with high accuracy \cite{Priv_EMGFeatDis, Priv_EMGPersIdentModels}. Collectively, these findings confirm that EMG signals contain persistent physiological signatures that are uniquely and reliably linked to a specific subject.

Beyond identity disclosure, EMG signals also facilitate more advanced inference attacks. Because forearm EMG captures fine motor mechanics of the hand, it also acts as a biological keylogger \cite{Priv_KeyloggingSideAttack}, with recent work reconstructing typed passwords with over 91\% accuracy \cite{Priv_EMG2PWD}. 
Given that participants frequently express concern regarding the potential for record linkage to reveal sensitive health conditions to third parties \cite{Priv_MomonaPT}, evaluating whether FL can obscure these user-specific EMG signatures is a critical step toward securing the next generation of wearable and neural interfaces.
}

\subsection{What is Federated Learning?}

Federated learning (FL) is a type of \textit{distributed learning}, where clients collaboratively train their models while keeping their raw data local (i.e., on device). 
Specifically, a set of decentralized clients (e.g., users, nodes, etc.) communicates with a coordinating server to optimize a shared global model.
FL strikes a balance between \textit{centralized learning} (high performance but high privacy risk due to data aggregation on a central server) and \textit{local learning} (low privacy risk but limited performance due to small datasets) \cite{tang2024distributed}.
We provide a brief overview of FL for readers unfamiliar with FL. 
Knowledgeable readers may want to skip this section and return as needed.
Refer to McMahan et al. \cite{FedAvg} or Fallah et al. \cite{Per-FedAvg} for an in-depth overview of FL.

The canonical FL formulation, FedAvg \cite{FedAvg}, optimizes a global model $w$ by minimizing the cost functions of $K$ users. 
For FedAvg, the global cost function $F(w)$ is the sum of all user $i$ cost functions $f_i(w)$: 
%
\begin{equation} \label{eqn:canonical_fl}
     \min_{w \in \mathbb{R}^d} F(w) = \frac{1}{K} \sum^K_{i=1} f_i(w)
\end{equation}
%
which optimizes for a model that performs well on average for all users.
%In each round, the server sends the current global model $w$ to a random subset of users. Each selected user performs several steps of gradient descent using their local data.
%The server waits for all users to upload their model updates before aggregating them via a weighted averaging scheme.
%
Variants such as FedProx~\cite{FedProx} and SCAFFOLD~\cite{SCAFFOLD} add regularization terms to reduce client drift, ensuring that local models stay close to the global one. These extensions aim to improve convergence under non-Independent and Identically Distributed (non-IID) conditions, which are common in biosignals \cite{Amy_CLDA_SkillfulNeuroProsCtrl, EMGHetero_EMGPatterns, EMGHetero_MultiSubj, EMGHetero_Norm}.

In neural interface applications, it is often desirable to personalize decoders to individual users.
Personalization can be incorporated into FL by shifting the optimization focus from a single shared model to user-specific models, optimizing for each user’s individual performance while retaining some shared learning or initialization via the global model.
One popular approach is Per-FedAvg \cite{Per-FedAvg}, which leverages Model-Agnostic Meta-Learning (MAML) to find a global initialization that is highly adaptable. Rather than optimizing a static global model $w$ directly (as in Equation \ref{eqn:canonical_fl}), the objective is to find a set of parameters that performs well after a small number of local gradient updates:
\begin{equation} \label{eqn:MAML}
\min_{w \in \mathbb{R}^d} F(w) = \frac{1}{K} \sum^K_{i=1} f_i(w - \alpha \nabla f_i(w))
\end{equation}
By minimizing this meta-loss, Per-FedAvg ensures that the shared global model serves as an effective prior, allowing individual users to rapidly personalize their models with minimal local computation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=1.5\columnwidth]{Figures/ML_Spectrum.png}
%   \caption{Personalization-privacy spectrum of machine learning approaches that illustrates the ideal scenarios for centralized learning (left), distributed learning (middle), and local learning (right). The user personalization and privacy increase as learning transitions from Centralized to Distributed to Local (i.e., from left to right). 
%   % Our work focuses on developing a framework for understanding the effects of Distributed Learning on performance and privacy.
%   }
%   \label{fig:ML_Spectrum}
% \end{figure*}

% \section{Federated Learning Background -- REMOVE THIS SECTION? Replace with the other one below}

% \subsection{What is Federated Learning?}

% Federated learning (FL) is a type of \textit{distributed learning}, where users collaborate through a central coordinating server to optimize a shared global model while keeping their raw data local (i.e., on device). 
% In comparison to \textit{centralized learning}, where all users upload their data to a central server to train a single model, or \textit{local learning}, where each user trains their own model, FL strikes a balance between privacy and performance by enabling local training (keeping raw data private) with coordinated model updates (model weights are aggregated across many users) \cite{tang2024distributed}.
% Centralized and local learning can be considered opposite ends of this performance-privacy trade-off (Fig.~\ref{fig:ML_Spectrum}).
% In centralized learning, data is not private since it must be uploaded to the server, where the user no longer has control or knowledge of how it is used (for example, if the server is breached or untrustworthy). The centralized model can often achieve high performance due to the scale of the dataset, but it is inherently a one-size-fits-all model and may be limited in neural interface applications where models can struggle to generalize across users.
% On the other hand, in local learning, raw data is not shared, but model performance may be limited because of the much smaller dataset.
% Furthermore, every user is burdened with training their own model from scratch. 
% FL offers an option between these extremes, where users do not have to give up custody of their data but still benefit from data in the network of users, enabling more generalizable models.

% In FL, each \textit{user} (also called client, agent, or node) communicates with the server via \textit{edge devices} of limited computational capacity \cite{adv_op_fl}. 
% The server does not access user data, but instead aggregates the users' model parameters into the \textit{global model} that solves the server's global cost function.
% %The server has the following properties: 1) does not have access to any user data, 2) often has more powerful hardware than the users, and 3) coordinates the users to solve the global cost function. 
% The global cost function represents an aggregated optimization objective that combines individual user cost functions, often incorporating weighting, regularization, or fairness constraints to improve generalization across distributed data sources.
% In FL, in addition to the server's global model, each user maintains their own set of model weights referred to as their \textit{local model}.

% \subsection{A Basic FL Algorithm}

% The canonical FL formulation, introduced in the FedAvg algorithm by \cite{FedAvg}, is a distributed setting in which $K$ users collaborate to find a set of global model weights $w$ that minimizes the global cost function. 
% In this work, we refer to such FL algorithms that aim to train a single shared global model for all users as \textit{traditional federated learning (TFL)}.
% For FedAvg, the global cost function $F(w)$ is the sum of all user cost functions $f_i(w)$: 
% %
% \begin{equation} \label{eqn:canonical_fl}
%      \min_{w \in \mathbb{R}^d} F(w) = \frac{1}{K} \sum^K_{i=1} f_i(w)
% \end{equation}
% %
% which optimizes for a model that performs well on average for all users $i$.
% In each round, the server sends the current global model $w$ to a random subset of users. Each selected user performs several steps of gradient descent using their local data:

% \begin{equation} \label{eqn:stochastic_fl}
%     w_i^{(t)} = w_i^{(t-1)} - \alpha\nabla f_i(w_i^{(t-1)}; \xi_i^t),
% \end{equation}
% % 
% where $\xi_i^t$ is a mini-batch of user $i$'s data at time $t$, $\alpha$ is the learning rate, and $\nabla$ indicates the gradient of cost function $f_i$.
% The server waits for all users to upload their updated local models before aggregating the uploaded models via a weighted averaging scheme.
% %
% Variants such as FedProx~\cite{FedProx} and SCAFFOLD~\cite{SCAFFOLD} add regularization terms to reduce client drift, ensuring that local models stay close to the global one. These extensions aim to improve convergence under non-IID conditions, which are common in biosignal data \cite{Amy_CLDA_SkillfulNeuroProsCtrl, EMGHetero_EMGPatterns, EMGHetero_fMRI, EMGHetero_MultiSubj, EMGHetero_Norm, EMGHetero_QTRR}.

% In neural interface applications, it is often desirable to personalize decoders to individual users.
% Personalization can be incorporated into FL by shifting the optimization focus from a single shared model to user-specific models, optimizing for each user’s individual performance while still allowing for some form of shared learning or initialization via the global model.
% One popular approach is Per-FedAvg~\cite{Per-FedAvg}, which draws from Model-Agnostic Meta-Learning (MAML). Rather than optimizing the global model $w$ directly (as in Equation \ref{eqn:canonical_fl}), Per-FedAvg optimizes for a model that performs well after one or a few gradient updates on each user’s data:
% %
% \begin{equation} \label{eqn:MAML}
%     \min_{w \in \mathbb{R}^d} F(w) = \frac{1}{K} \sum^K_{i=1} f_i(w - \alpha \nabla f_i(w)),
% \end{equation}
% %
% Thus, MAML optimizes for a global model that is a good starting point for its users, such that users can quickly personalize, regardless of whether the global starting point model achieves strong performance.
% This allows users to quickly personalize the shared model without needing to train from scratch, balancing the benefits of shared learning with user-specific adaptation.

% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=1\columnwidth]{Figures/FedAvgIllustration.jpg}
%   \caption{Visualization of the steps involved with one training round of the FedAvg algorithm. In general, FL distributes the training computation across client devices, communicating only the model parameters.}
%   \label{fig:FedAvgIllustration}
%   %\Description{Graphic illustration of the federated learning training process, divided into 5 steps. The first step shows how the server samples a subset of clients, sending each selected client a copy of its global model weights. The second step depicts each of the selected clients training the received global model weights, using their own datasets. Step 3 shows each selected client uploading their now-trained local model weights back to the server. Step 4 shows the server aggregating all the uploaded model weights, averaging all the uploaded model weights to set the next round's global model weights. Step 5 shows this process repeating, this time with a new subset of clients.}
% \end{figure}
% %\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/sec_framework.tex <==
\section{FL for Privacy-Preserving Neural Interfaces}
Applying federated learning (FL) to neural interfaces presents unique challenges, particularly due to the myriad of available FL algorithms and the complex demands of real-time neural systems. 
In this section, we introduce a conceptual framework to help researchers reason about FL in offline and online neural decoding and other biosignal-based scenarios.
Whereas existing frameworks (e.g., Flower \cite{flower}) look to provide the code for simulating FL algorithms, our framework focuses on guiding researchers' choice of FL algorithm for their application.
Rather than recommending a single specific algorithm, our goal is to highlight two key attributes that influence the applicability and performance of FL in neural interface studies: (1) personalized cost and (2) user availability. 
Understanding these attributes can help practitioners identify potential pitfalls and necessary algorithmic adjustments when implementing FL in privacy-sensitive neural interface applications (see Table~\ref{tab:FL_algos_wSUS}).

\subsection{Attribute 1: Personalized Cost}

FL algorithms are broadly categorized into traditional (TFL) and personalized (PFL) based on their optimization objectives. The primary driver for this selection is the data heterogeneity inherent in the problem, which dictates whether a single global model can sufficiently represent the diverse data distributions across all users. If the variance across users is high, a traditional global model may incur a high personalized cost, leading to significant performance degradation for individual participants compared to a model tailored to their specific data distributions. In practice, this heterogeneity is rarely explicitly measured; instead, researchers often rely on domain expertise to judge dataset heterogeneity and whether personalization is necessary.

\subsubsection{Traditional Federated Learning (TFL)}
TFL algorithms, such as FedAvg \cite{FedAvg}, focus on training a single, shared global model that performs well for all users. 
When all users sample from the same distribution (i.e., data across users are relatively homogeneous), the global model benefits from a large multi-user dataset, leading to improved performance. 
In comparison, training a local (i.e., non-federated) model for each user is limited to the smaller single-user dataset, which can hinder performance and generalization, and each new user must train their local model from scratch.
In the presence of substantial data heterogeneity, TFL often suffers from slow or unstable convergence and degraded performance~\cite{APFL}. 
Although some TFL variants attempt to accommodate heterogeneity~\cite{heterogeneous_fl_sota, heterogeneous_fl_learn_from_others}, the FL research community has increasingly shifted toward PFL approaches.

\subsubsection{Personalized Federated Learning (PFL)}
PFL algorithms can be grouped into two categories: those addressing device heterogeneity (e.g., network reliability and hardware capabilities) and those addressing data heterogeneity. In this work, we concentrate on the latter.
PFL optimizes a set of user-specific models tailored to each user's data distribution, often using the global model as a prior or initialization to improve generalization and stability. These approaches are made to be more robust to distributional variation but are often more complex to tune and slower to converge~\cite{PersAFL}. 
If dataset heterogeneity is unknown, personalized models may offer a more robust solution, trading faster convergence for better performance.
A growing number of PFL algorithms address diverse personalization scenarios, including Per-FedAvg~\cite{Per-FedAvg}, pFedMe~\cite{pFedMe}, APFL~\cite{APFL}, FedALA~\cite{FedALA}, Fedcp~\cite{Fedcp}, FedDBE~\cite{FedDBE}, and GPFL~\cite{GPFL}, with many works benchmarked on standardized image datasets such as CIFAR-100 \cite{CIFAR100}.

\begin{table*}[!t]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{
Categorization of FL algorithms based on relevant dimensions (see Zhang \cite{tsingz0} for a large but non-comprehensive list, with PyTorch code). 
Although new FL algorithms often outperform older ones on specific tasks/datasets, it is difficult to know which algorithm will perform best for an arbitrary task/dataset. 
% This table serves as a flexible reference, helping researchers categorize both existing and future FL algorithms for their specific applications.
}
\label{tab:FL_algos_wSUS}
\begin{tabular}{c c c}
\hline
\textbf{Dimension 1: Personalized Cost} & \textbf{Dimension 2: User Availability} & \textbf{Example Algorithms} \\
\hline
Traditional & Synchronous & FedAvg \cite{FedAvg}, FedProx \cite{FedProx}, FedDyn \cite{FedDyn}, FedNTD \cite{FedNTD} \\
Personalized & Synchronous & Per-FedAvg \cite{Per-FedAvg}, pFedMe \cite{pFedMe}, FedALA \cite{FedALA}, GPFL \cite{GPFL}, FedDBE \cite{FedDBE}\\
Traditional & Asynchronous & FedAsync \cite{FedAsync}, FedSA \cite{FedSA}, AsyncDrop \cite{HAsyncDrop} \\
Personalized & Asynchronous & PersA-FL-MAML \cite{PersAFL}, PersA-FL-ME \cite{PersAFL}, Hetero AsyncDrop \cite{HAsyncDrop} \\
\hline
\end{tabular}
\end{table*}

\subsection{Attribute 2: User Availability}
User availability refers to how frequently and reliably user information can be integrated back into the network. 
This includes real-world issues such as users dropping out of the network, differences in computational resources, and variations in network connection speeds (e.g., delays). Our framework considers three modes of user availability: synchronous, asynchronous, and sequential. 

\subsubsection{Synchronous}
Synchronous FL assumes that all users are available simultaneously. This is the default assumption for most FL algorithms ~\cite{FedAvg, FedALA, FedDBE, FedDyn, FedProx, pFedMe, Per-FedAvg}.
While simple and easy to simulate, synchronous FL has limited applicability to laboratory-based, online neural interface experiments, where running multiple users simultaneously is often infeasible due to hardware or personnel constraints.
Looking towards deployment, synchronous FL also struggles with straggling users that require substantially more time: slow users delay the entire training process, and users unexpectedly dropping out of the network can halt training indefinitely~\cite{FL_straggler}.
Synchronous algorithms are often sufficient for offline simulations, where real-time latency, hardware, and personnel constraints do not apply.

\subsubsection{Asynchronous}
Asynchronous FL relaxes the requirement of simultaneous user availability.
Typically, users can query the server at their own pace, thus reducing sensitivity to stragglers and dropouts \cite{PersAFL}. 
However, this flexibility introduces new challenges. First, updates from slower users may be based on outdated global models, leading to ``stale'' updates relative to the current global model. Second, faster users can dominate the training process, introducing bias (i.e., over-representation) into the global model. 
More recent algorithms address these issues through fairness and weighting mechanisms~\cite{IMWUTFL_AreYouLeftOut_Fair, IMWUTFL_BiasMitigation}.
Asynchronous methods offer a more robust alternative to synchronous FL, particularly for real-world deployment. However, asynchronous approaches still assume a small group of concurrently active users. 
This ongoing stream of diverse updates is key, as it serves as implicit regularization, helping prevent overfitting to any single user.
% , which more recent algorithms have worked to address \cite{IMWUTFL_AreYouLeftOut_Fair, PersAFL}.
%Asynchronous FL algorithms are uncommon and frequently have "A" or "Asynchronous" in their name \cite{PersAFL}. 

\subsubsection{Sequential}

We introduce a novel learning scenario we term \textit{sequential federated learning}, defined by two constraints: (1) only one user is active at a time, and (2) each user appears exactly once, fully completing their training during this window. 
This regime is highly relevant for online decoding experiments, such as EMG or brain-computer interface (BCI) studies \cite{ELEC677_EMGNeuralMachineInterface, ELEC677_UnsupTrackingLatentManifolds, ELEC677_FuncReorgBoMI, ELEC677_GaitResponseAnkleExo, ELEC677_PersExo}, where participants contribute data in isolation, and repeated access to a given user is uncommon outside of larger-scale longitudinal studies. 
Despite its practical importance, no existing FL algorithms are designed for this scenario.

Sequential FL breaks a core assumption of FL that updates from multiple users can be aggregated via averaging each training round. 
Since only one client is active per round, averaging-based model aggregation becomes model replacement: the global model is overwritten with the (sole) active user's uploaded model. 
This diminishes the stabilizing effect of averaging over users, increasing the likelihood of overfitting to the active user. 
Furthermore, if a user's model drifts far from the current global model, this can exacerbate client drift and hinder convergence. 
When users are seen only once, mitigating overfitting to individual users becomes critical. 
%Techniques such as early stopping~\cite{Early_Stopping}, regularization, or memory-based approaches like elastic weight consolidation~\cite{EWC} may help, but these have not been studied in this setting.

Although no prior work addresses this exact setting, a few related paradigms exist. 
For instance, \textit{cyclical FL}~\cite{CyclicFL, CyclicFL_Medical} also assumes one user trains at a time but relaxes the single-pass constraint by returning to previous users in a cyclical fashion. 
This approach is often applied in the institutional context, with a small number of persistent institutions that pass the model weights around in a continuous cycle, thus violating the second constraint of our sequential FL definition.
%Finally, we note that “sequential FL” has appeared in prior literature~\cite{FedFMC, NIPS_SeqFL, DataPos_SeqFL}, but with different, unrelated meanings ~\cite{FedFMC, NIPS_SeqFL, DataPos_SeqFL}. 
%Depending on the paper, it can refer to 1) the stepwise application of algorithmic components~\cite{FedFMC}, 2) the sequential nature of the data (i.e., time series and adjacent data types), or 3) how clients are processed (i.e., sequential versus parallel) within synchronous FL training rounds~\cite{NIPS_SeqFL, DataPos_SeqFL}. 
%Our definition of sequential FL refers instead to a unique client availability regime, motivated by the realities of neural interface studies and other online neural experiments.
In summary, our formulation of sequential FL introduces unique challenges not addressed by prior work, motivating the development of new methods for real-world online neural applications.


==> sections/sec_intro.tex <==
\section{Introduction}
\label{sec:introduction}

\IEEEPARstart{N}{eural} interfaces enable human-centric, accessible, and high-bandwidth inputs~\cite{wheelchair_gestures, MomonaDisUBGestures, Shenoy_bimanual_BCI, Shenoy_speech_BCI}.
Machine learning models (i.e., \textit{decoders}) play a crucial role in this process, translating high-dimensional neural signals into device inputs \cite{IMU_HAR, CV_GestureCustomization, CTRL_Labs, TNSRE_AttentionEEGMotorImageryDecoding, TNSRE_EMGAttention}.
% However, their efficacy depends on large quantities of biosignal data and burdensome calibration procedures. 
% This data is often scarce due to its task-specific, user-dependent nature and inherent privacy risks \cite{Priv_MomonaPT, Priv_MorrisAIAccess}.
However, high-dimensional neural signals can reveal sensitive attributes such as identity~\cite{Priv_EEGPersonIdentification, Priv_GaitPersonIdentification}, age~\cite{Priv_ECGAgeSexEstimation}, and sex~\cite{Priv_ECGAgeSexEstimation} during decoder training.
This makes individuals hesitant about contributing data and institutions cautious about open-sourcing datasets~\cite{Priv_HiddenInfoInBios, Priv_KeyloggingSideAttack, Priv_BiosensingInPublic}.
This creates a fundamental tension between the data needs for training decoders and the desire for user privacy~\cite{PPP_BigData, PPP_Survey, PPP_AttentionEcon, PPP_Smartphone, PPP_LocAwareMark, PPP_transparency, PPP_OG06}.
Federated learning (FL) offers a solution by enabling distributed training in which users train models locally and share only model updates rather than their raw neural data, eliminating the need to transmit or store sensitive neural signals centrally.

\rev{Despite its potential, applying FL to co-adaptive neural interfaces remains a significant and unexplored frontier. While FL has been extensively studied in simulated or offline settings \cite{FLwBioS_EpilepSeizPred, FLwBioS_SleepStagingEEG, FLwBioS_MitigateThreatsEEG, FLwBioS_EvoEEG, TNSRE_FL_MotorImageryClsBCI, TNSRE_FL_CerebellarAtaxia}, its application to online neural interfaces \cite{Orsborn_CLDA, CPHS, CL_CoAdaptation_DynamicMyoelectricInterface, NeuralFeedback_BMI, CL_FPGA_Spikesorting, CL_Ctrl_FES, CL_DBS} introduces unique challenges that arise when federated optimization is integrated into a real-time, online training environment. Unlike traditional FL research that focuses on aggregation across static, pre-recorded datasets, these online interfaces often involve human-decoder co-adaptation, where the user and decoder influence each other through continuous interaction \cite{CPHS, CL_CoAdaptation_DynamicMyoelectricInterface}. This dynamic introduces a critical gap: co-adaptive behaviors and real-time latency constraints may destabilize FL optimization in ways that are entirely absent in offline work. For instance, FL hyperparameters optimized in offline simulation may prove infeasible during real-time user interactions.

To address this gap, we provide the first empirical evaluation of FL in a live user study, moving beyond offline simulation to identify where standard FL assumptions break down in online training environments. Beyond performance, we explore a critical re-identification risk, demonstrating that subject identity can be recovered directly from persistent decoder weights even in the absence of raw neural data.

To facilitate future research in this nascent application, we propose a high-level framework that characterizes the inherent properties and trade-offs of different FL algorithm categories. We evaluate this framework by adapting Per-FedAvg for sequential training and comparing high-dimensional EMG decoding across offline (i.e., simulated) and online (i.e, real-time) scenarios. Our results highlight how the transition from offline simulation to online interaction alters the relationship between personalization and privacy, providing a starting point for algorithms specifically tuned for closed-loop decoder adaptation dynamics.
}

==> sections/sec_method.tex <==
\section{Methods}
\label{sec:methods}

The goal of our empirical evaluation is to analyze how decoder performance and privacy risk vary not only across learning strategies (i.e., local learning versus FL) but also across two key settings for high-dimensional neural interface control: offline and online control. By running matched experiments under both conditions, we assess how learning paradigms generalize and adapt in offline versus online decoding scenarios.
In particular, in our online user study, we analyze closed-loop decoder adaptation (CLDA), in which the decoder’s parameters are updated continuously during interaction to accommodate changes in the user’s neural (myoelectric) signals. This process creates a dynamic, co-adaptive relationship in which the user modifies their motor strategy in response to the decoder's performance, and simultaneously, the FL algorithm optimizes the model weights to track the user's shifting physiological patterns.
%Given the success shown with online adaptation~\cite{Orsborn_CLDA}, we expect online convergence to be influenced by this human-interface co-adaptation process~\cite{madduri2024predicting}.

\subsection{Task and Adaptive Decoder Description}

The offline study is a secondary data analysis of the data collected in Madduri et al. \cite{CPHS}, and the online study experiment adapts the same task of Madduri et al. \cite{CPHS} to facilitate direct comparison.
Briefly, subjects were asked to control a cursor $y$ in the horizontal and vertical directions on the screen to track a reference $r$ using an EMG interface placed on their forearm (Fig.~\ref{fig:setup}). 
The reference trajectory was the sum of two sinusoids with frequencies 0.10 and 0.25 Hz in the horizontal direction and 0.15 and 0.35 Hz in the vertical direction, each starting each trial with a random phase to prevent trajectory memorization. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/Hardware_Picture.jpg}
    \caption{Experimental setup. The subject controls a blue cursor using their forearm muscles, with activity recorded from a 64-channel Quattrocento EMG sensor. The subject's goal is to track the red target by minimizing the distance between the blue cursor and the red reference trajectory.}
    \label{fig:setup}
    %\Description{A photo of a man sitting at a desktop computer with their arm on an armrest. The computer has a 2D trajectory tracking task consisting of a large red circle and a smaller blue circle on a black screen, and the man has wired surface EMG electrodes just below his elbow secured with red athletic tape. There is a closeup picture in the top right corner of the figure showing the EMG electrodes without the red athletic tape obscuring them, and a legend explaining that the larger red circle on the computer screen is the target and the smaller blue circle is the subject-controlled cursor.}
\end{figure}

\subsubsection{EMG Data Collection and Filtering}
EMG data were collected using the Quattrocento system (Bioelettronica, Italy), measuring the dominant hand's forearm muscle activity with a 64-channel electrode array (5×13 electrode layout). All subjects were right-handed.
EMG data was collected at 2048 Hz and filtered via built-in analog high- and low-pass filters at 10 Hz and 130 Hz, respectively.
We then computed the EMG linear envelope following~\cite{Momona_EMG}, and applied a rolling average with a window size of 250 ms and 93\% overlap to downsample the EMG data from 2048 Hz to 60 Hz.
% https://github.com/kdmalc/labgraph-Rice/blob/b5eb55ef3def570d004ab0f805ca4090f277a982/experiment/nodes/emg_inputs.py#L184

\subsubsection{EMG-to-Cursor Decoder and Adaptation}

Detailed methods and decoder parameter analysis can be found in~\cite{CPHS}.
Briefly, linear regression was used to convert the streamed EMG data
($s\in\mathbb{R}^{64\times 1}$) into the $x$ and $y$ cursor velocity ($v=w s$, where $w \in\mathbb{R}^{2\times 64}$ are the decoder parameters and $v\in\mathbb{R}^{2\times 1}$).
The cursor velocity $v$ was numerically integrated to obtain the horizontal and vertical cursor positions. 
The decoder parameters $w$ were updated in roughly 20-second batches by minimizing the sum of the squared difference between the velocity error and the magnitudes of the decoder parameters. The velocity error is defined as the difference between the decoder's predicted velocity and the optimal gap-closing velocity between the reference $r$ and the user's cursor $y$ velocities:
%
\begin{equation}\label{eq:cost_func}
    \min\limits_{w} f(w) = ||w s - \frac{\partial}{\partial t}(r-y)||_2^2 + \lambda||w||_2^2,
\end{equation}
%
where $\lambda_{w}$ is the penalty parameter associated with the L2 norm on the decoder parameters $w$.
All decoder updates implemented SmoothBatch~\cite{Orsborn_CLDA}, where the optimal decoder parameters are linearly combined with the old decoder parameters $w_{new} = (1-\alpha) w_{old} + \alpha w_{optimal}$, with learning rate $\alpha$.
In line with prior work~\cite{CPHS}, our pilot online studies found that a penalty parameter of $\lambda=10^{2}$ and a slow SmoothBatch learning rate of $\alpha=0.75$ performed well; hence, these were used in our offline and online studies. 
The dataset collected by Madduri et al. \cite{CPHS} was an online experiment, but did not use FL: rather, each subject trained their own local decoder using what we refer to as the \textit{\CPHSAlgo{}} algorithm. 
Each subject started with random initial decoder parameters and adapted simultaneously with the decoder during each 5-minute trial. 

\subsection{Choosing an FL Algorithm: Applying Attributes to Determine Suitability}

We used Table \ref{tab:FL_algos_wSUS} for our offline and online EMG decoding to identify possible FL algorithms using the two attributes: personalized cost and user availability. 

\subsubsection{Offline Study}

% In our offline study, we would like to implement both PFL and TFL algorithms to compare their performance.
For the first attribute, \textit{personalized cost}, we use our domain expertise to estimate the dataset's heterogeneity. 
It is well known that many types of neural signals are highly unique and heterogeneous \cite{Amy_CLDA_SkillfulNeuroProsCtrl, EMGHetero_EMGPatterns, EMGHetero_fMRI, EMGHetero_MultiSubj, EMGHetero_Norm, EMGHetero_QTRR}. Thus, for high-dimensional neural interfaces, we can assume the dataset is heterogeneous.
This would lead us to focus on PFL algorithms. However, we would like to use the offline study to investigate whether PFL or TFL algorithms perform best in our specific domain; thus, we will implement both a TFL and a PFL algorithm.
For the second attribute, \textit{user availability}, our offline study (i.e., simulation) provides full control over user availability, as we can set the constraints.
Thus, we chose to simulate the standard synchronous case, where all users are available at the same time.
Considering the results of both dimensions, we accept any synchronous TFL and PFL algorithms, corresponding to rows 1 and 2 in Table \ref{tab:FL_algos_wSUS}.
% Considering the results of both dimensions, we highlight the algorithms that meet our minimum criteria in Table \ref{tab:FL_algos_wSUS}.
%
For PFL algorithms, we have no prior on which PFL algorithm (e.g., Per-FedAvg, pFedMe, etc.) will perform best on our dataset; thus, we implement Per-FedAvg as a baseline based on its popularity in other works \cite{FedDBE, GPFL, Fedcp, PFLBridging, PFL_SharedReprs, PFL_FirstOrder}. 
Likewise for TFL algorithms, from the acceptable Table \ref{tab:FL_algos_wSUS} row 1 algorithms, we choose to implement FedAvg for our case studies, as this is the original FL algorithm and thus a good starting point and baseline for researchers new to FL. 
%
% Thus, we implement our baseline \CPHSAlgo{} algorithm (not federated, not part of the framework), FedAvg, and Per-FedAvg, which are traditional non-federated machine learning, traditional FL, and personalized FL, respectively.

\subsubsection{Online Study}

For the first attribute, \textit{personalized cost}, we assume the dataset is heterogeneous and therefore best suited to a PFL algorithm. 

For the second attribute, \textit{user availability}, when running online studies in the lab environment, we are constrained to using a single data-acquisition device, so only one participant can participate in the experiment at a time. 
This necessitates a sequential FL setup, where users train one at a time and do not return for subsequent rounds. However, no such algorithms exist.
Thus, we use our framework to determine which algorithm to start with.
Since we are not constrained by real-world deployment challenges such as stragglers or intermittent connectivity, we do not require the robustness offered by asynchronous FL methods.
Therefore, we adapt an existing synchronous FL algorithm for the sequential setting. 
This allows us to preserve algorithmic simplicity while accommodating only the necessary constraints of our online, real-time experiment.

Taking the results of both attributes into consideration, the algorithms of row 2 in Table \ref{tab:FL_algos_wSUS} satisfy these attributes.
Given the proliferation of Per-FedAvg as a baseline ~\cite{pFedMe, GPFL, DITTO, FedDBE, FedALA} and our desire to match our offline study, we chose Per-FedAvg over the other PFL algorithms.

\subsection{Adaptive Algorithm Implementation}

We implemented a baseline non-federated algorithm (\textit{\CPHSAlgo{}}) and two FL algorithms (\textit{Per-FedAvg} and \textit{FedAvg}) for the offline study and a \textit{Local} and FL algorithm (modified \textit{Per-FedAvg}) for the online study.~\footnote{The code is available at https://github.com/kdmalc/framework-for-fl-emg}

\subsubsection{Local}
We implemented the same \textit{Local} learning algorithm used in prior work~\cite{CPHS}, where Equation~\ref{eq:cost_func} is minimized using the Python package \texttt{scipy.minimize()}. 
We ran SmoothBatch \cite{Orsborn_CLDA} between the user's current decoder weights and the new optimal decoder weights to ensure that the decoder does not change too drastically for the user.
This algorithm is subject-specific, using only the data from the subject's most recently streamed update.
In both the offline and online studies, \CPHSAlgo{} fully minimized each streamed update, with each update comprising 20 seconds of data.

\subsubsection{Per-FedAvg and Sequential Modification}
\textit{Per-FedAvg} optimizes the MAML cost function (Eq. \ref{eqn:MAML}). For both the offline and online implementations, we implemented first-order Per-FedAvg, approximating the Hessian with a first-order term.

In the offline study, Per-FedAvg was run for 500 global rounds, selecting 35\% of clients per round and performing 25 gradient steps per client. 
Each client advanced to their next streamed update after completing 25 local training rounds, meaning clients progressed at different rates due to the random sampling of clients each round.
Once a client advanced to the final streamed update, they used it for the rest of the simulation.

In the online study, we ran 40 training rounds on each streamed update, with 20 seconds of data per update. We divided each update into 6 batches to achieve real-time speed.
To accommodate the sequential nature of our human-subject study, we modified the original Per-FedAvg algorithm \cite{Per-FedAvg} by replacing the standard multi-user averaging scheme with a weighted average between the active subject’s updated weights and the server's current global weights. 
In our linear implementation, this modification is mathematically equivalent to SmoothBatch regularization \cite{Orsborn_CLDA}, which constrains the local decoder to remain in proximity to the global parameters. 
Although this approach removes simultaneous cross-user averaging, the global model still serves as a shared, evolving initialization that is passed between participants, effectively linking sequential local learning optimizations through a shared global prior.

\subsubsection{FedAvg} 
%The FedAvg algorithm is the baseline algorithm for FL, coming from the paper that first introduced FL \cite{FedAvg}. 
FedAvg is implemented only for the offline study and shares all of Per-FedAvg's described hyperparameters, with the only difference being the cost function it optimizes (Eq. \ref{eqn:canonical_fl}).

%[!t]
\begin{table*}[tb]
\centering
\caption{\rev{Comparison of offline and online evaluation settings.}}
%\caption{Comparison of offline and online evaluation settings.}
\begin{subtable}{0.48\textwidth}
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Offline (Synchronous, N=14)}
\begin{tabular}{c c c c}
\hline
Algorithm & Eval. Scenario & Model Init. \\
\hline
\CPHSAlgo{} \cite{CPHS} & Intra-Subj. & Random \\
\CPHSAlgo{} \cite{CPHS} & Cross-Subj. & Random \\
FedAvg \cite{FedAvg} & Intra-Subj. & Random \\
FedAvg \cite{FedAvg} & Cross-Subj. & Random \\
Per-FedAvg \cite{Per-FedAvg} & Intra-Subj. & Random \\
Per-FedAvg \cite{Per-FedAvg} & Cross-Subj. & Random \\
\hline
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}{0.48\textwidth}
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Online (Sequential, N=16)}
\begin{tabular}{c c c c}
\hline
Algorithm & Eval. Scenario & Model Init. \\
\hline
\CPHSAlgo{} \cite{CPHS} & Intra-Subj. & Random \\
\CPHSAlgo{} \cite{CPHS} & Intra-Subj. & Offline \\
Static & Intra-Subj. & Pretrained \\
Modified Per-FedAvg & Intra-Subj. & Random \\
Modified Per-FedAvg & Intra-Subj. & Offline \\
\hline
\end{tabular}
\end{subtable}
\end{table*}

\subsection{Outcome Measures}

Our primary outcomes for both the offline and online studies were 1) \textit{Velocity Error} and 2) \textit{Model Re-identification Risk}. 
These outcomes compare each decoder's performance and privacy risk across the tested FL algorithms.

\subsubsection{Velocity Error}
We quantified decoder performance using velocity error, which is equivalent to an unscaled version of the first term of the user cost function:
\begin{equation}\label{eq:vel_error}
    v_e = ||w s - \frac{\partial}{\partial t}(r-y)||_2^2 
\end{equation}
The last full decoder update was used to evaluate each user's test performance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Model Re-identification Risk}

\rev{In our threat model, we assume the raw EMG data remains on the user device and is never directly at risk. However, we assume an adversary may intercept the communicated model weights or access leaked model weights via a server-side breach. 
Inspired by recent works taking advantage of gradient leakage \cite{DLG, Priv_FedACDP_DLG} as well as foundational works in record linkage attacks \cite{Priv_LINDDUN, Priv_KAnon}, we quantified Model Re-identification Risk as the ability (i.e., accuracy) of an adversarial classifier to infer subject identity from trained decoder weights. 
High identification accuracy suggests that the trained decoder weights encode subject-specific information, potentially increasing vulnerability to more advanced attacks commonly conducted against deep learning models (e.g., membership inference~\cite{MemInfAttack} or model inversion~\cite{ModelInvAttack}). 
We distinguish this specific technical metric, which measures the linkability of model weights to individuals, from broader user privacy concerns, such as the explicit disclosure of sensitive health conditions to third parties \cite{Priv_MomonaPT} or model inversion attacks \cite{ModelInvAttack}.
}

\rev{We conducted our adversarial attack on the decoder weights rather than gradients for two reasons. First, the FL algorithms explored in this study (FedAvg and Per-FedAvg) both communicate model weights rather than gradients, thereby making the model weights vulnerable during distributed training. Second, while gradients are typically not stored, model weights are necessarily stored and often backed up, representing a more persistent threat model in both Local and FL settings. In particular, for models trained solely on-device (i.e., our non-federated Local models), the gradients are never extracted or communicated, thus making gradient-based attacks unrealistic. Moreover, gradients typically leak more information than weights \cite{DLG}; thus, our approach provides a conservative lower bound of the re-identification risk.}

To evaluate this privacy risk, we extracted a representative set of decoder snapshots from each user and condition. 
Specifically, we selected the final six decoder updates per user (i.e., the final six streamed updates, by which point the model should have been sufficiently trained), ensuring consistency across conditions. We flattened these decoder snapshots into vectors and assembled them into comprehensive datasets covering all subjects.
We then performed leave-one-sample-out cross-validation to quantify the adversary's ability to correctly identify subjects from their decoder weights. 
For each sample, we trained a support vector classifier (SVC) on all other samples and assessed whether the model correctly identified the held-out sample's subject identity. By aggregating these predictions over all iterations, we obtained a per-subject accuracy measure, reflecting each subject's Model Re-identification Risk.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Offline Evaluation and Analysis}

\subsubsection{Dataset}

The offline evaluation presented here used only the data from the best-performing condition from Madduri et al. \cite{CPHS}: a slow (SmoothBatch) learning rate ($\alpha=0.75$), a low decoder parameter penalty ($10^{2}$), and a positive decoder parameter initialization. 
In total, each trial consisted of five minutes of data for each of the 14 subjects.
Because we did not simulate the subjects' changing EMG responses to adaptive decoders, we excluded the initial two updates (of 18 total) to allow initial learning and adaptation effects to stabilize. Thus, our analysis used data from update three onward (approximately 4 minutes of the 5-minute trial duration).%, resulting in roughly 17,000 time points per subject.

\subsubsection{Data Streaming and Train/Test Split}

In the data-collection experiment, each subject's data was streamed in 18 consecutive updates, each containing 20 seconds of data. 
To replicate this streaming effect in our offline study, we segmented the dataset so that the decoder trains on one update at a time. After training for a predefined number of rounds, the simulated subject advances to the next update in the sequence.

\begin{figure}[htbp]
  \centering
  %,trim={1cm 2cm 4cm 2cm},clip]
  \includegraphics[width=1\columnwidth]{Figures/IntraVsCrossScenarios.jpg}
  \caption{Offline data splits: \CPHSAlgo{} train (blue), FL train (grey), and test (orange) split for the first fold in seven-fold cross-validation ($N=14$ subjects). 
  For the \textit{Intra-Subject Scenario}, the federated decoder is trained across six training folds for all 14 subjects.
  Each subject-specific \CPHSAlgo{} decoder is trained on a single subject's six training folds and evaluated on that subject's withheld testing fold.
  For the \textit{Cross-Subject Scenario}, the federated decoder is trained on the entire dataset for Subjects 1-12, and cross-subject decoders are evaluated on Subjects 13-14. Likewise, the \CPHSAlgo{} decoders are trained on a single subject's data, and all are tested on the same withheld subjects.}
  \label{fig:IntraVsCrossScenarios}
  %\Description{A table showing two scenarios for training machine learning decoders. Both scenarios are shown as rows of 5 rectangles labeled by subject number for each row (subjects 1-14). Rectangles are colored blue for the train set and orange for a test set, and there is a larger grey rectangle enclosing the blue rectangles to represent the federated train set. On the left, there is a section labeled "Intra-Subject Fold 1". In this section, each subject (1-14) has 4 blue rectangles for the train set and 1 orange rectangle for the test set. All of the blue rectangles are encircled by a grey rectangle representing the federated train set. On the right, there is a section labeled "Cross-Subject Fold 1". Subjects 1-11 have all blue rectangles for the train set, and those blue rectangles are all encircled by a grey rectangle representing the federated train set. Subjects 12-14 have all orange rectangles, representing the test set.}
\end{figure}

\subsubsection{Evaluation Design}

% The primary reported outcomes for all conditions were Tracking Error and Empirical Privacy Risk. 
The offline evaluation was performed with the following factors and levels:
%
\begin{itemize}[leftmargin=*]
    \setlength\itemsep{0em}
    \item \textit{Algorithm} (within-subject): Local, Per-FedAvg, FedAvg;
    \item \textit{Scenario} (within-subject): Intra-Subject, Cross-Subject.
\end{itemize}
%
We evaluated two \textit{Scenarios}: Intra-Subject and Cross-Subject. For both scenarios, we followed a k-fold cross-validation test/train split with k=7.
In the \textit{Intra-Subject Scenario}, we implemented a data split within each user, with some of their data withheld for the final outcome evaluation.
Each subject's dataset is divided into seven folds, with one fold held out as the test set during each evaluation (Fig.~\ref{fig:IntraVsCrossScenarios}, left). 
In the \textit{Cross-Subject Scenario}, we tested decoders on data from withheld subjects that were not included in the training dataset.
Here, we implemented a user-based data split by randomly assigning subjects to seven groups. For each fold, one group was used as the testing subjects and the other six groups were used as the training subjects (Fig.~\ref{fig:IntraVsCrossScenarios}, right). 

\subsubsection{Statistical Analysis}

For the offline studies, we found that the residuals from a $2\times 2$ within-subjects factorial repeated-measures ANOVA model for the dataset were highly non-normal. 
Therefore, we performed a rank transformation on the outputs~\cite{conover1981rank} and found that the residuals of the transformed ANOVA model were normally distributed (Kolmogorov-Smirnov test: $p>0.05$). 
Holm's sequential Bonferroni procedure~\cite{holm1979simple} was used to correct for multiple comparisons when performing \textit{post-hoc} tests on significant main and interaction effects.

\subsection{Online Evaluation and Analysis}

Our protocol was approved by Rice University's Institutional Review Board (IRB-FY2024-3) on August 28th, 2023; informed consent was obtained from all participants. 

\subsubsection{Real-Time Implementation}
In our online study, we used batches of 20 seconds, as pilot studies found that this was optimal for FL's stability. Thus, over the roughly five-minute trial, we had 15 updates. 
The reference tracking task, real-time EMG streaming, and decoder parameter adaptation were implemented in \texttt{Python3} using LabGraph \cite{LabGraph}. %~\cite{https://github.com/facebookresearch/labgraph}.

\subsubsection{Subject Demographics}
16 people (8 women, 8 men) participated in the study. 
Subjects were all right-handed (61\% all dominant, 39\% somewhat ambidextrous in handedness), with an average weight and standard deviation of 151.1 ± 36.8 lbs, a height of 65.9 ± 3.6 in, a forearm circumference of 10.1 ± 1.1 in, and an age of 23 ± 2 years. All subjects were daily computer users.

\subsubsection{Evaluation Design}

The online evaluation was performed with the following factors and levels:

\begin{itemize}[leftmargin=*]
    \setlength\itemsep{0em}
    \item \textit{Algorithm} (within-subject): Local, Per-FedAvg, Static;
    \item \textit{Initialization} (within-subject): Random, Simulation. 
\end{itemize}
%
For \textit{Algorithm}, in addition to \textit{\CPHSAlgo{}} and \textit{Per-FedAvg}, subjects also completed a ``Static'' condition, where they used their previously trained \textit{\CPHSAlgo{}} decoder, but during this trial, no further decoder training happened. This provides a baseline of how subjects learn and adapt to fixed decoders without co-adaptation.
We initialized the Static condition using subject-specific, previously trained \CPHSAlgo{} decoders, rather than a generic global decoder or one pre-trained on either offline simulations or an expert EMG user, because subjects could not gain control with these decoders during pilot testing. 

We evaluated two \textit{Initializations} for \CPHSAlgo{} and Per-FedAvg: Random and offline. 
In the \textit{Random Initialization} condition, the decoder weights were randomly generated as positive values between 0 and 1; all subjects used the same set of weights.
In the \textit{Offline Initialization} condition, all clients started from the final Per-FedAvg global decoder from our offline study. 

To minimize learning and fatigue effects, trial orders were randomized for each subject, following a Latin Square design. 

\subsubsection{Statistical Analysis}

For the online studies, we found that the residuals from a $2\times 2$ within-subjects factorial repeated-measures ANOVA model for the dataset were highly non-normal. 
Therefore, we performed a rank transformation on the outputs~\cite{conover1981rank} but found that the residuals of the transformed ANOVA model were still not normally distributed (Kolmogorov-Smirnov test: $p<0.0005$). 
Thus, we ran an aligned rank transform (ART) ANOVA to fit a nonparametric factorial repeated-measures model. 
We also performed planned paired Wilcoxon signed-rank tests comparing Static with all other conditions.
The Holm's sequential Bonferroni procedure ~\cite{holm1979simple} was used to adjust for multiple comparisons. 

\subsection{Offline and Online Decoder Analysis}

We analyzed the convergence of decoders in two ways: first, for each trial, we took the Euclidean distance between each decoder and that trial's final decoder. Second, we flattened all decoders, mean-subtracted them, and then used PCA projections to visualize them in a two-dimensional subspace.

